Beyond Textual Issues: Understanding the Usage and Impact of GitHub Reactions

Recently, GitHub introduced a new social feature, named reactions, which are "pictorial characters" similar to emoji symbols widely used nowadays in text-based communications. Particularly, GitHub users can use a pre-defined set of such symbols to react to issues and pull requests. However, little is known about the real usage and impact of GitHub reactions. In this paper, we analyze the reactions provided by developers to more than 2.5 million issues and 9.7 million issue comments, in order to answer an extensive list of nine research questions about the usage and adoption of reactions. We show that reactions are being increasingly used by open source developers. Moreover, we also found that issues with reactions usually take more time to be handled and have longer discussions.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

(TODO)
